Collaborative Filtering Bandits

Classical collaborative filtering, and content-based filtering methods try to learn a static recommendation model given training data. These approaches are far from ideal in highly dynamic recommendation domains such as news recommendation and computational advertisement, where the set of items and users is very fluid. In this work, we investigate an adaptive clustering technique for content recommendation based on exploration-exploitation strategies in contextual multi-armed bandit settings. Our algorithm takes into account the collaborative effects that arise due to the interaction of the users with the items, by dynamically grouping users based on the items under consideration and, at the same time, grouping items based on the similarity of the clusterings induced over the users. The resulting algorithm thus takes advantage of preference patterns in the data in a way akin to collaborative filtering methods. We provide an empirical analysis on medium-size real-world datasets, showing scalability and increased prediction performance (as measured by click-through rate) over state-of-the-art methods for clustering bandits. We also provide a regret analysis within a standard linear stochastic noise setting.

==> experiments2.tex <==

\section{Experiments}\label{s:exp}
We compared our algorithm to standard bandit baselines on three real-world datasets: one canonical benchmark dataset on news recommendations, one advertising dataset from a living production system, and one publicly available advertising dataset. In all cases, no features on the items have been used. We closely followed the same experimental setting as in previous work
%and evaluated the predication performance with the click-through rate as d
~\cite{chu2011contextual,glz14}, so that we evaluated prediction performance by click-through rate.


\subsection{Datasets}

\textbf{Yahoo.} The first dataset we use for the evaluation is the freely available benchmark dataset which 
was released in the ``ICML 2012 Exploration \& Exploitation Challenge"\footnote{https://explochallenge.inria.fr/category/challenge}. The aim of the challenge was to build state-of-the-art news article recommendation algorithms on Yahoo! data, by building an algorithm that learns efficiently a policy to serve news articles on a web site. 
%The evaluation metric used in the challenge CTR (click through rate). 
The dataset is made up of random traffic records of user visits on the ``Today Module'' of Yahoo, implying that both the visitors and the recommended news article are selected randomly. 
%The dataset contains user visits on the Yahoo! news website. 
The available options (the items) correspond to a set of news articles available for recommendation, one being displayed
in a small box on the visited web page. The aim is to recommend an interesting article to
the user, whose interest in a given piece of news is asserted by a click on it. 
The data has $30$ million visits over a two-week time stretch. Out of the logged information contained in each record, 
we used the user id in the form of a $136$-dimensional boolean vector containing his/her features (index $i_t$), the
set of relevant news articles that the system can recommend from (set $C_{i_t}$); a randomly recommended article during the visit; a boolean value indicating whether the recommended article was clicked by the visiting user or not (payoff $a_t$). 
Because the displayed article is chosen uniformly at random from the candidate article pool, one can use an unbiased off-line evaluation method to compare bandit algorithms in a reliable way.
We refer the reader to ~\cite{glz14} for a more detailed description how the dataset was 
collected and extracted. We picked the larger of the two datasets considered in \cite{glz14}, resulting in
$n \approx 18K$ users. The number of records was $2,829,308$, out of which we took the first $300,000$ for parameter tuning 
and the rest for testing. 
% The computation resource we utilised for this dataset is one Mac laptop with $2.6$GHz Intel Core i5 and $8$GB RAM.
We carried out offline policy evaluation by only retaining the records on which the logged policy recommendation did coincide with the one issued by the algorithms we tested. Because records are discarded on the fly, the actual number of retained records changes slightly across algorithms, but it is around 70K for all of them. 





\textbf{Telefonica.} This dataset was obtained from Telefonica S.A., which is the number one Spanish broadband and 
telecommunications provider with businesses units in Europe and South America etc. This data contains clicks on ads displayed to user on 
one of the websites that Telefonica operates. The data was collected from the backend server logs.  
 This data consists of two files: One containing the ads interactions, each record contains an impression timestamp, a user-ID, an action, the ad type, order item ID, click timestamp ; the second file contains the ads metadata as item-ID, type-ID, type, order-ID, creative type, mask, cost, creator-ID, transaction key, cap type. 
The number of users are in the million scale, while the number of items is approximately 300. The data contains $15,479,561$ records. 
We took the first $1,500,000$ records as the training and the rest for testing. 
The only available payoffs are those associated with the items served by the system, in order to make the 
procedure be an effective estimator in a sequential decision process (e.g.,~\cite{cgz13,cg11,dudik12,glz14,li2010contextual}), we simulated the random 
choices by the system by setting the available item sets $C_{i_t}$ as follows: 
at each round $t$, we stored the ad served to the current user $i_t$
and the associated payoff value $a_t$ (1 =``clicked", 0 =``not clicked"). Then we created 
$C_{i_t}$ by including the served ad along with $9$ extra items (hence $c_t = 10$ $\forall t$) which 
were drawn uniformly at random in such a way that, for any item $\be_j \in \scI$, if $\be_j$ occurs in some set 
$C_{i_t}$, this item will be the one served by the system $1/10$ of the times. The 
random selection was done independent of the available payoff values $a_t$. All the experiment on this data were run on 
a machine with $64$GB RAM and $32$ Intel Xeon cores.

\textbf{Avazu.} This dataset was prepared by Avazu Inc\footnote{https://www.kaggle.com/c/avazu-ctr-prediction} which is a leading multinational corporation in the digital advertising business. The data was provided for the challenge to predict the click-through rate of impressions on mobile devices, i.e., whether a mobile ad will be clicked or not. The number of samples is $40,428,967$, we took the first $4,000,000$ samples as the training set and remaining for testing. Each line in the data represents the event of an ad impression on the site or in a mobile application (app) along with additional context information. The payoff variable takes the value $1$ if the user clicks on the ad, and $0$ otherwise. The data form for each sample is like the following: ad-ID; timestamp (date and hour); click (boolean variable); device-ID; device IP; connection type; device type; ID of visited App/Website; category of visited App/Website; connection domain of visited App/Website; banner position; anonymized categorical fields (C1, C14-C21). We pre-processed the dataset as follows: we cleaned the data by filtering out the records where there are existing missing values for their corresponding attributes, and then we removed the outliers. We made the inference that C14 is ad-ID, and we identified the user with device-ID if it is not null, in both cases of users and items the size level is in the millions scale. Here we constructed the recommendation list with length $20$ for each different timestamp using the same routine as described above. After that we feed the streaming data to our model as the input, and then deployed all the trained models. All the data are transferred to Amazon S3 and all the jobs are finished in the Amazon Web Services\footnote{Thanks to the Amazon AWS Award in Large Scale Machine Learning Research Grant}, the EC2 instance we chose is the one ``Ubuntu Server 14.04 LTS (HVM), SSD Volume Type - ami-33db9803''  and ``r3.8xlarge'' in Oregon region.

\subsection{Algorithms}
%
We compared {\sc COFIBA} to a number of competitors: 
\begin{itemize}
%\vspace{-0.03in}
\item {\sc LINUCB-ONE}~\cite{chu2011contextual} is a single instance of the {\sc ucb1}~\cite{ACF01} algorithm, which is very popular and achieved 
dramatical researcher's attention since then;
\item {\sc DYNUCB} is the dynamic {\sc ucb} algorithm of~\cite{nl14}. This algorithm adopts a ``$K$-means''-like 
clustering technique so as to dynamically re-assign the clusters on the fly based on the changing 
contexts and user preferences over time;
\item {\sc LINUCB-IND}~\cite{cgz13} is a set of independent {\sc ucb1} instances, one per user, which provides the fully personalised recommendation for each user;
%\vspace{-0.04in}
\item {\sc CLUB}~\cite{glz14} is the state-of-the-art online clustering of bandit algorithm that dynamically cluster users based on the confidence 
ellipsoids of their models; 
%\vspace{-0.04in}
\item {\sc LINUCB-V}~\cite{audibert:hal-00711069} is also a single instance of the {\sc ucb1}~\cite{ACF01} but with more sophisticated confidence bound which was the 1st Golden Championship Winner of ``ICML 2012 Challenge'' as mentioned above
%\vspace{-0.04in}
\end{itemize}
%

We tuned the optimal parameters in the training set with standard grid search as indicated in~\cite{cgz13,cg11,glz14}, and used the test set to evaluated the predictive performance of the algorithms. Since the system's recommendation need not coincide with the recommendation issued by the algorithms we tested, we could only retain the records on which the two recommendations were indeed the same. Because records are discarded on the fly, the actual number of retained records changes across algorithms, is about $70,000$ for the Yahoo! data, $350,000$ for the Telefonica data, and $900,000$ for the Avazu data. All experimental results reported were averaged over $3$ runs, in fact the variance we observed is quite small.


